On the Existence of Envy-Free Allocations Beyond Additive Valuations

We study the problem of fairly allocating $m$ indivisible items among $n$ agents. Envy-free allocations, in which each agent prefers her bundle to the bundle of every other agent, need not exist in the worst case. However, when agents have additive preferences and the value $v_{i,j}$ of agent $i$ for item $j$ is drawn independently from a distribution $D_i$, envy-free allocations exist with high probability when $m \in \Omega( n \log n / \log \log n )$. In this paper, we study the existence of envy-free allocations under stochastic valuations far beyond the additive setting. We introduce a new stochastic model in which each agent's valuation is sampled by first fixing a worst-case function, and then drawing a uniformly random renaming of the items, independently for each agent. This strictly generalizes known settings; for example, $v_{i,j} \sim D_i$ may be seen as picking a random (instead of a worst-case) additive function before renaming. We prove that random renaming is sufficient to ensure that envy-free allocations exist with high probability in very general settings. When valuations are non-negative and ``order-consistent,'' a valuation class that generalizes additive, budget-additive, unit-demand, and single-minded agents, SD-envy-free allocations (a stronger notion of fairness than envy-freeness) exist for $m \in \omega(n^2)$ when $n$ divides $m$, and SD-EFX allocations exist for all $m \in \omega(n^2)$. The dependence on $n$ is tight, that is, for $m \in O(n^2)$ envy-free allocations don't exist with constant probability. For the case of arbitrary valuations (allowing non-monotone, negative, or mixed-manna valuations) and $n=2$ agents, we prove envy-free allocations exist with probability $1 - \Theta(1/m)$ (and this is tight).

==> SDEF_2_agents.tex <==
\section{Monotone Valuations}

\begin{theorem}
With $2$ agents, even $m$, and agent orders selected uniformly at random, Round Robin is sd-EF with probability $1 - \Theta(1/\sqrt{m})$.    
\end{theorem}
\begin{proof}
    We begin with a lower bound on this probability. For agent $1$, they always sd-prefer their own bundle. So we consider the perspective of agent $2$. From their perspective, this process is equivalent to their item ordering being fixed $g_1 \succ \cdots \succ g_m$ and at each round agent $1$ takes a uniformly random selected remaining item. We upper bound the probability the final allocation is not sd-preferred at the $k$'th item. By union bounding over all $k \le m/2$, we get an upper bound on the probability of the entire allocation violating sd-EF (and thus a lower bound on the probability that the allocation is sd-EF).
    
    Fix some $k$. Let $G^\ell = \set{g_1, \ldots, g_\ell}$ be agent $2$'s top $\ell$ items. Let $A^k_1$ and $A^k_2$ be agent $2$'s top $k$ items in the bundls $A_1$ and $A_2$. Notice that agent $2$'s $k$'th most preferred item they will receive will be at least as good as $g_{2k}$. In other words, $A^k_2 \subseteq G^{2k}$. Hence, the only way agent $1$'s will have a better $k$'th best good is if theirs is $g_\ell$ for $\ell \le 2k - 1$, i.e., $A^k_1 \subseteq G^{2k - 1}$. For this to happen, all of the first $k$ picks must have been from the top $G^{2k - 1}$ items. Notice that this is not only necessary, but actually a sufficient condition. We can directly analyze the probability of this occuring. 
    
    We have that all of agent $2$'s first $k - 1$ picks will be from $G^{2k - 1}$ because at least one must be available. Hence, when agent $1$ makes the $\ell$'th pick for $\ell \le k$, conditioned on them always taking an item from $G^{2k - 1}$ before hand, there will be $2k - 1 - 2(\ell - 1)$ items from $G^{2k - 1}$ remaining. This is out of a total of $m - 2(\ell - 1)$ items. Hence, the total probability of this occuring ate very step for $\ell$ from $1,\ldots, k$ is
    \[
    	\frac{2k - 1}{m} \cdot \frac{2k - 3}{m - 2} \cdot \cdots \cdot \frac{1}{m - 2(k - 1)} = \frac{(2k - 1)!!}{m!!/(m - 2k)!!}.
    \]
    Using the known identities $(2\ell)!! = 2^\ell \ell!$ and $(2\ell - 1)!! = \frac{(2\ell)!}{(2\ell)!!} = \frac{(2\ell)!}{2^\ell \ell!}$, we can simplify this to
    \[
    	\frac{(2k)!}{2^k k!} \cdot \frac{(m/2 - k)!2^{m/2 - k}}{(m/2)! 2^{m/2}} = \frac{1}{2^{2k}} \frac{(2k!)}{k!} \cdot \frac{(m/2 - k)!}{m!} = \frac{1}{2^{2k}} \frac{(2k!)}{k!k!} \cdot \frac{(m/2 - k)!k!}{m!} = \frac{\binom{2k}{k}}{2^{2k}} \frac{1}{\binom{m/2}{k}}.
    \]
    For upperbounding, we can use the fact that $\frac{\binom{2k}{k}}{2^{2k}} \le \frac{1}{\sqrt{k}}$,\footnote{\url{https://math.stackexchange.com/questions/1442351/stirling-approximation-of-binom2nn}} so this value is at most $\frac{1}{\sqrt{k}}\frac{1}{\binom{m/2}{k}}$.
    
    We now union bound over all $k \le m/2$, that is, we want to show $\sum_{k = 1}^{m/2} \frac{1}{\sqrt{k} \cdot \binom{m/2}{k}} \in O(1/\sqrt{m})$. Indeed, notice that for $k = m/2$, this value is $\frac{1}{\sqrt{m/2}}$. For $k = 1$ and $k = m/2 - 1$, this value is at most $\frac{2}{m}$. For $2 \le k \le m-2$, this value is at most $\frac{1}{\binom{m/2}{2}} \le \frac{2}{(m/2)(m/2 - 1)}$. There are at most $m - 3$ of these values, so we have that adding up over all terms,
    \[
    	\sqrt{\frac{2}{m}} + 2\frac{2}{m} + \frac{2(m/2 - 3)}{m/2(m/2 - 1)} \le \frac{\sqrt{2}}{\sqrt{m}} + \frac{8}{m} \in O(1/\sqrt{m}),
    \]
    as needed. For an upperbound, we can use the fact that $\frac{\binom{2k}{k}}{2^{2k}} \ge \frac{1}{2\sqrt{k}}$, which implies that with probability at least $1 - \frac{1}{\sqrt{2m}}$, for $k = m/2$, the bundle will not be preferred.
\end{proof}
The above proof suggests a better method for getting sd-EF. We simply want to avoid having a bad probability for $k = m/2$. Notice that this only occurs if an agent gets their least preferred item. Hence, instead, consider \emph{give-away-RR} where in the first step, agent $1$ gives agent $2$ their least preferred item, then agent $2$ gives agent $1$ their least-preferred remaining item, and from this we continue with RR. We then have the following.
\begin{theorem}
	With $2$ agents, even $m$, and agent orders selected uniformly at random, give-away-RR is sd-EF with probability $1 - \Theta(1/m)$.
\end{theorem}
Notice that this is asymptotically optimal because with probability $1/m$, the two agents have the same top item so no sd-EF allocation can exist.
\begin{proof}
	Notice that give-away-RR is still deterministically sd-EF for agent 1, so we only consider agent 2. We do the same analysis as for RR. For $k = m/2$, the probability is just $1/m$, as it is simply the probability agent $1$ gives agent $2$ $g_m$.
	
	Consider $k < m/2$. We will do a similar analysis to RR. Notice that agent $2$ will never give agent $1$ a good in $G^{2k - 1}$ in the first step (at least one of $g_{m}$ and $g_{m - 1}$ must be available), although it is possible that agent $1$ gives agent $2$ a good from $G^{2k - 1}$. Either way, agent 2's $k$'th best good will be at least as good as $g_{2k}$, so it must be the case that all of agent $1$'s first $k$ picks came from $G^{2k - 1}$. Notice that if agent $1$ gives agent $2$ an item from $G^{2k - 1}$, this is actually impossible because agent $2$ is able to guarantee $k$ items from $G^{2k - 1}$ (so if agent $1$ also has $k$ then $|G^{2k - 1}|$ would need to be at least $2k$). So, we can compute this probability as
	\[
		\left(1 - \frac{2k - 1}{m} \right) \cdot \frac{2k - 1}{m - 2} \cdot \frac{2k - 3}{m - 4} \cdot \cdots \cdot \frac{1}{m - 2(k - 1) - 2} = \left(1 - \frac{2k - 1}{m} \right) \frac{(2k - 1)!!}{(m - 2)!!/(m - 2 - 2k)!!}.
	\]
	The above analysis tells us that
	\[
		\frac{(2k - 1)!!}{(m - 2)!!/(m - 2 - 2k)!!} = \frac{\binom{2k}{k}}{2^{2k}}\frac{1}{\binom{m/2 - 1}{k}},
	\]
	For this portion, we can use the weaker bound of $ \frac{\binom{2k}{k}}{2^{2k}} \le 1$ to get an upper bound of 
	\[
		\frac{m - 2k + 1}{m} \frac{1}{\binom{m/2 - 1}{k}}.
	\]
	For $k = m/2 - 1$, this is $3/m$. For $k = 1$ and $k = m/2 - 2$, we can use the same bound  as before to get $\frac{1}{m/2 - 1} = \frac{2}{m - 2}$. For all other $m/2 - 4$ values we get an upper bound of $\frac{2}{(m/2 - 1)(m/2 - 2)}$. This gives us a total probability of
	\[
		\frac{1}{m} + \frac{3}{m} + \frac{2 \cdot 2}{m - 2} + \frac{2(m/2 - 4)}{(m/2 - 1)(m /2 - 2)} \in O(1/m),
	\]
	as needed.
\end{proof}

==> SDEF_n_agents.tex <==
We can now generalize the RR proof to $n$ agents.

\begin{theorem}
    With $n$ agents and $m = q \cdot n$ (i.e., divisible by $n$), Round Robin is sd-EF with probability at least $1 - O\left(\frac{n^2\log m}{m^{\frac{n - 1}{n}}}\right)$.
\end{theorem}
\begin{proof}
    Notice that lower index agents never envy higher index agents. We will show that for all $j < i^*$, the probability that $i^*$ envies $j$ is at most $O\left(\frac{ \log m}{m^{\frac{n - 1}{n}}}\right)$. The result will follow by a union bound over all $\binom{n}{2}$ choices of $i^*$ and $j$.
    
    Fix such an $i^* > j$. Fix an ordering of the goods (from the perspective of $i^*$), $g_1 \succ \cdots \succ g_m$ \alex{do we need to discuss ties?}. We will again fix some specific $k \le m/n = q$ and upper bound the probability $i^*$ envies $j$ on the $k$'th item. The analysis for $k < q$ will be quite different from $k = q$. 
    
    We first focus on $k < q$.   Recall that from $i^*$'s perspective, at each of the other agent's picks, they take a uniformly at random selected item from the ones remaining, and on $i^*$'s pick, they take the best item remaining. We let $P_{i\ell}$ be the random variable for the index of the good picked in agent $i$'s $\ell$'th pick. We let $R_{t}$ be the random variable denoting the set of indexes of the goods remaining after $t$ picks (so $|R_t| = m - t$). We also use the notation $R^{(r)}_t$ for the $r$'th best good available in $R_t$. %This means that $R_0$ is simply the entire set of goods. 
    For $i \ne i^*$, $P_{i\ell} | R_{(\ell - 1)n + (i - 1)}$ is a uniformly at random selected good in $R_{(\ell - 1)n + (i - 1)}$. For $i^*$, $P_{i^*\ell}|R_{(\ell - 1)n + (i^* - 1)}$ is $R_{(\ell - 1)n + (i^* - 1)}^{(1)}$ (i.e., this is deterministic) as $i^*$ always takes the best remaining good. Notice that $i^*$ will only envy $j$ on the $k$'th good if $P_{j\ell} < P_{i^*k}$ for all $\ell \le k$.
    
    Notice that between any two of $i^*$'s selections, these samples are just independent uniform samples, so they form a (uniformly) random subset. This makes it clear that it does not matter what order the picks happen (we could instead imagine sampling the $n - 1$ items that will be picked and after randomly assign them to the picking agents). Hence, it is without loss of generality to assume that in this process, $j = i^* - 1$, i.e., $j$ picks directly before $i^*$.  \daniel{Justify this more}
    
    Fix some $\ell \le k$ and consider the remaining goods $R_{(\ell - 1)n + (j - 1)}$ when $j$ is making their $\ell$'th pick. Notice that $i^*$ will be making their $k$'th pick exactly $n(k - \ell) + 2)$ picks from now. This implies that $P_{i^*k} \le R^{(n(k - \ell) + 2)}_{(\ell - 1)n + (i^* - 1)}$. In words, $i^*$ is guaranteed a good at least as good as the $(n(k - \ell) + 2)$'th best remaining one. This is because at least one of these top ones will be available at that time.
   This also implies that if $i^*$ is going to envy $j$, then it must be the case that $j$ chose a better item, i.e.,  $P_{j\ell} < R^{(n(k - \ell) + 2)}_{(\ell - 1)n + (j - 1)}$. This occurs exactly when $P_{j\ell} = R_{(\ell - 1)n + (j - 1)}^{(r)}$ for $r \le n(k - \ell) + 1$. Let $E_\ell$ be the event that this occurs.
   
   Notice that $\Pr[E_{\ell}] = \frac{n(k - \ell) + 1}{|R_{(\ell - 1)n + (j - 1)}|}$ since $P_{j\ell}$ is a uniformly selected item from $R_{(\ell - 1)n + (j - 1)}^{(r)}$. Further, for $i^*$ to envy $j$ on the $k$'th item, all of $E_1, \ldots E_{k}$ must occur. Additionally, all these events are independent as the random selections are independent. 
    
    Hence, putting this toegether, we have that
    \begin{align*}
    	\Pr[i^* \text{ envies } j \text{ on the } k\text{'th item}]
    	&\le \Pr\left[\bigcap_{\ell = 1}^k E_\ell\right]\\
    	&= \prod_{\ell = 1}^k \Pr[E_\ell]\\
    	&= \prod_{\ell = 1}^k\frac{n(k - \ell) + 1}{|R_{(\ell - 1)n + (j - 1)}|}\\
    	&= \prod_{\ell = 1}^k\frac{n(k - \ell) + 1}{m - ((\ell - 1)n + (j - 1))}\\
        &=\prod_{\ell = 1}^k \frac{(k - \ell)n + 1}{(q + 1 - \ell)n - (i^* - 2)}\\
        &= \prod_{\ell = 1}^k \frac{(k - \ell)n + 1}{(q - \ell)n + (n - i^* + 2)}\\
        &\le \prod_{\ell = 1}^k \frac{(k - \ell)n + 1}{(q - \ell)n + 1}\\
        &= \prod_{\ell = 1}^k \frac{k - \ell + 1/n}{q - \ell + 1/n}\\
        &= \frac{\Gamma(k + 1/n)}{\Gamma(1/n)} \cdot \frac{\Gamma(q - k + 1/n)}{\Gamma(q + 1/n)}\\
        &= \frac{1}{\Gamma(1/n)} \frac{\Gamma(k + 1)\Gamma(q - k +1)}{\Gamma(q + 1)}\cdot \frac{\Gamma(k + 1/n)}{\Gamma(k + 1)}\cdot \frac{\Gamma(q - k + 1/n)}{\Gamma(q - k + 1)}\cdot \frac{\Gamma(q + 1)}{\Gamma(q + 1/n)}\\
        &< \frac{1}{\Gamma(1/n)} \cdot \frac{1}{\binom{q}{k}} \frac{1}{k^{1 - 1/n}}\frac{1}{(q - k)^{1 - 1/n}}(q + 1)^{1 - 1/n}\\
        &= \frac{1}{\Gamma(1/n)}\frac{1}{\binom{q}{k}} \left(\frac{q + 1}{k(q - k)}\right)^{1 - 1/n}\\
        &< \frac{1}{\Gamma(1/n)}\frac{1}{\binom{q}{k}} \left(\frac{2q}{q/2}\right)^{1 - 1/n}\\
        &\le \frac{1}{\Gamma(1/n)}\frac{1}{\binom{q}{k}} 4^{1 - 1/n}\\
        &= O\left(\frac{1}{n\binom{q}{k}}\right)
    \end{align*}
    where the ninth transition follows by the gamma representation of falling factorial, the eleventh by Gautchi's inequality, the thirteenth by the fact that $q + 1 \le 2q$ and at least one of $k$ and $(q - k)$ are at least $q/2$, and the last because $\Gamma(1/n) \in \Omega(n)$.\footnote{\url{https://en.wikipedia.org/wiki/Particular_values_of_the_gamma_function}}
    As before, summing up over all $1 \le k \le q - 1$ gives $O(\frac{1}{nq}) = O(\frac{1}{m})$. 
    
    Next, we consider $k = q$. We begin by showing this for $i^* = n$  and describe how to modify the argument for $i^* < n$ later. To do this, we begin by bounding the probability that $i^*$ receives an extremely bad item on their last pick. For a fixed $r \le m$, let $E_r$ be the event that $P_{qn} = r$, that is, agent $n$ picks $g_r$ on their very last pick. For this to happen, $r$ must \emph{not} be picked in any of the first $m - 1$ timesteps. Since $\Pr[r \text{ is available at timestep } 1] = 1$ (all items are available at the beginning), we can write this as \[ \Pr[E_r] = \prod_{t = 1}^{m - 1} \Pr[r \text{ is not picked at timestep } t \mid r \text{ is available at timestep } t].\]
    Although $\Pr[r \text{ is not picked at timestep } t \mid r \text{ is available at timestep } t]$ when agent $i^*$ is picking is hard to compute and depends on $r$,  for all others, it is very easy. Since other agents are picking random available items, it is simply $\frac{m - t}{m + 1 - t}$. Hence, we can upper bound the product by ignoring non multiple of $n$ terms (they are always at most $1$) to get a bound of
    \[\prod_{t = 1:n \nmid t}^m \frac{m - t}{m - t + 1} = \frac{\prod_{t = 1}^m\frac{m - t}{m - t + 1}}{\prod_{t = 1: n \mid t}^m \frac{m - t}{m - t + 1}} = \frac{(m - 1)!}{m!} \prod_{t=1:n \mid t}^m \frac{m - t + 1}{m - t} = \frac{1}{m} \prod_{\ell = 1}^q \frac{q - \ell + 1/n}{q - \ell} = \frac{1}{m}\frac{(1/n)^{(q)}}{(q - 1)!}
    \]
    where $(1/n)^{(q)}$ represents the rising factorial. Converting this to gamma function representations, this is
    \[
    \frac{1}{m} \frac{\Gamma(q + 1/n)}{\Gamma(1/n)\Gamma(q)}.
    \]
    We have that $\Gamma(1/n) \in \Omega(n)$ and by Gautchi's inequality,  $ \frac{\Gamma(q + 1/n)}{\Gamma(q)} < (q + 1/n)^{1/n} = (m+1)^{1/n}/n^{1/n} \in O(m^{1/n})$. Together, these imply that this probability is at most $O(\frac{1}{n\cdot m^{(n - 1)/n}})$.
    
    Since $\Pr[E_r] \in O(\frac{1}{n\cdot m^{(n - 1)/n}})$, $\Pr[\bigcup_{r = m - 3n\log m}^m E_r] \in O(\frac{\log m}{m^{(n - 1)/n}})$; in words, the probability that agent $n$ gets any of their bottom $3n \log m$ items in their final pick is at most $O(\frac{\log m}{m^{(n - 1)/n}})$. We now show conditioned on this, agent $n$ does not envy agent $j$ with probability at least $1 - O(1/m)$. This implies a total failure probability of at most $O(\frac{\log m}{m^{(n - 1)/n}}) + O(1/m) = O(\frac{\log m}{m^{(n - 1)/n}}).$
    
    To that end, we can imagine of instead giving each agent each item for every pick, we sample a subset of $n - 1$ non-agent-$n$ picks and and only at the end decide which agent received which of these picks in every round. We now condition on $q$ $(n-1)$-subsets $R_1, \ldots R_q$ and $q$ agent-$n$ picks $p_1, \ldots, p_q$ such that $p_q < m - 3n\log m$, i.e., agent $n$'s final pick was better than $g_{m - 3n \log m}$. Since $p_1 < \cdots p_q$, this implies that agent $n$ did not receive any of their final $3n\log m$ items, and they must all be contained in the subsets $R_1, \ldots R_q$. We now sample which item in each of the subsets $R_1, \ldots R_q$ will be agent $j$'s and we are interested in the probability that $j$ gets at least one of the final $3n\log m$ items. If this occurs, then agent $n$ will prefer their worst item to agent $j$'s worst item, so will not envy $j$ in the $k = q$ position. Suppose $R_\ell$ has $r_\ell$ such items. Notice that the probability $j$ gets one of these is $r_\ell / (n - 1)$ and this is independent for each $\ell$. This is the sum of $q$ independent Bernoulli random variables with total expected value at least $3n\log m / (n - 1) \ge 3\log m$. Therefore a Chernoff bound says that the probability the sum is $< (1 - \delta) 3 \log m$ is at most $e^{-\delta^2 3 \log m / 2}$. By choosing  $\delta > \sqrt{2/3}$, we see that the probability the sum equals $0$ is at most $e^{-\log m} = 1/m$, as needed.
    
    \emph{Extending to other agents:} We wish to upper bound the probability that each agent $> 1$ receives an item from their bottom $4n \log m$. Consider the $i$'th-from-last agent $n + 1 - i$. Notice that the only way they receive such an item is that on their last pick, when $i$ items are available, all $i$ are one of these bottom items. Let $E^{r_1, \ldots, r_i}$ be the event that on their last pick they are left with goods $r_1, \ldots, r_i$.  By union bounding over all $\binom{4n\log m}{i}$ choices of these goods contained in the last $4n\log m$, we can upper bound the probability they are forced to choose such an item. For a specific set $r_1, \ldots, r_i$, at every timestep other than ones where $t \equiv n + 1 - i \pmod{n}$, the probability of all $i$ goods surviving is $\frac{m + 1 - t - i}{m + 1 - t}$. To avoid off-by-one errors, a more convenient way to think about this is by the number of items remaining, which we denote by $c$. When there are $c$ remaining, assuming it is not the envying agent's pick, the probability of not picking $r_1, \ldots, r_i$ is simply $\frac{c - i}{c}$. The value of $c$ should range from $i + 1$ all the way up to $m$. Further, $i$ picks whenever the number of remaining items is exactly equal to $i \pmod{m}$. That is, whenever $c$ is equal to $n\ell  + i$ for $\ell$ ranging from $1$ to $q - 1$.
    
    Hence, this probability is at most
    \begin{align*}
        \prod_{c = i + 1: c \not\equiv i}^m \frac{c - i}{c}
        &= \frac{\prod_{c = i + 1}^{m} \frac{c - i}{c}} {\prod_{c = i + 1: c \equiv n + 1 - i}^{m} \frac{c - i}{c}}\\
        &= \prod_{c = i + 1}^{m} \frac{c - i}{c} \cdot \prod_{c = i + 1: c \equiv n + 1 - i}^{m} \frac{c}{c - i}\\
        &= \frac{1}{\binom{m}{i}} \prod_{\ell = 1}^{q - 1} \frac{n \ell + i}{n \ell + i - i}\\
        &= \frac{1}{\binom{m}{i}} \prod_{\ell = 1}^{q - 1} \frac{\ell + i/n}{\ell}\\
        &= \frac{1}{\binom{m}{i}} \frac{\Gamma(q + i/n)}{\Gamma(1 + i/n)\Gamma(q)}\\
        &< \frac{2}{\binom{m}{i}}\left(\frac{m + i}{n}\right)^{i/n}
    \end{align*}
    where the last inequality holds because the Gamma Function has a global minimum on positive reals above $1/2$.
    
    Union bounding over the $\binom{4\log m}{i}$ possible choices of $r_1, \ldots, r_i$, we get an upper bound of \[
        2 \frac{\binom{4n \log m}{i}}{\binom{m}{i}} \left(\frac{m + i}{n}\right)^{i/n}.
    \]
    Using the fact that $\binom{4n \log m}{i} \le (4n\log m)^i$ and $\binom{m}{i} \ge (m - i)^i$, we can upper bound this with
    \[
        \le 2 \left( \frac{(4n \log m)(m + i)^{1/n}}{(m - i) n^{1/n}} \right)^i \le 2 \left( \frac{(4n \log m)(m + n)^{1/n}}{(m - n) n^{1/n}} \right)^i.
    \]
    Under the condition that $m \ge 2n$, we get that $(m - n) \ge m/2$, $(m + n)^{1/n} \le (2m)^{1/n} \le 2m^{1/n}$. Additionally using that $n^{1/n} \ge 1$, we have this is at most
    \[
        2 \left( \frac{16n \log m }{m^{1 - 1/n}} \right)^i.
    \]
    We will be union bounding over all $i$ ranging from $1$ to $n - 1$, i.e., we need to upper bound
    $2\sum_{i = 1}^{n - 1} \left( \frac{16n \log m }{m^{1 - 1/n}} \right)^i.$ However, as long as the $\frac{16n \log m }{m^{1 - 1/n}} \le 1/2$, this is at most
    \[
        4 \left( \frac{16n \log m }{m^{1 - 1/n}} \right) = \frac{64 n \log m}{m^{1 - 1/n}}.
    \]
    Hence, to get this sub constant, it is sufficient to choose $m \in \Omega(n^{1 + \varepsilon})$ for some $\varepsilon > 0$.
  \end{proof}

